S-DyRF: Reference-Based Stylized Radiance Fields for Dynamic Scenes

Current 3D stylization methods often assume static scenes, which violates the dynamic nature of our real world. To address this limitation, we present S-DyRF, a reference-based spatio-temporal stylization method for dynamic neural radiance fields. However, stylizing dynamic 3D scenes is inherently challenging due to the limited availability of stylized reference images along the temporal axis. Our key insight lies in introducing additional temporal cues besides the provided reference. To this end, we generate temporal pseudo-references from the given stylized reference. These pseudo-references facilitate the propagation of style information from the reference to the entire dynamic 3D scene. For coarse style transfer, we enforce novel views and times to mimic the style details present in pseudo-references at the feature level. To preserve high-frequency details, we create a collection of stylized temporal pseudo-rays from temporal pseudo-references. These pseudo-rays serve as detailed and explicit stylization guidance for achieving fine style transfer. Experiments on both synthetic and real-world datasets demonstrate that our method yields plausible stylized results of space-time view synthesis on dynamic 3D scenes.

==> sec/3_background.tex <==
\section{Background}
\label{sec:background}

\noindent\textbf{Neural radiance fields.}
Neural radiance fields~\cite{mildenhall2020nerf} are an implicit representation that maps a spatial location $\mathbf{x}=(x,y,z)$ and viewing direction $\mathbf{d}=(\theta,\phi)$ to its corresponding emitted color $\mathbf{c}$ and volume density $\sigma$: 
\begin{equation*}
    F_\Theta:(\mathbf{x},\mathbf{d}) \rightarrow (\mathbf{c}, \sigma),
\end{equation*}
where $F_\Theta$ is usually implemented with multilayer perceptrons (MLPs). The color $\hat{C}$ of a camera ray $\mathbf{r} = \mathbf{o} + t \mathbf{d}$ with near and far bounds $t_n$ and $t_f$ is given by:
\begin{gather}
    \hat{C}(\mathbf{r}) = \int_{t_n}^{t_f} T(t) \, \sigma(\mathbf{r}(t)) \, \mathbf{c}(\mathbf{r}(t), \mathbf{d}) \,dt, \nonumber\\
    \text{where} \ \  T(t) = \exp \left( -\int_{t_{n}}^{t} \sigma(\mathbf{r}(s)) \, ds \right).
\end{gather}
During the training phase, the neural radiance field is optimized by minimizing the difference between the predicted pixel colors $\hat{C}(\mathbf{r})$ and the ground truth pixel colors $C(\mathbf{r})$:
\begin{equation}
     \mathcal{L} = \sum_{\mathbf{r} \in \mathcal{R}} \Big\Vert \hat{C}(\mathbf{r}) - C(\mathbf{r}) \Big\Vert_2^{2}.
\end{equation}

\noindent\textbf{4D scene representation.}
A straightforward approach to representing dynamic 3D scenes is to condition the neural radiance fields on the timestamps~\cite{xian2021space,wang2021neural}. Nevertheless, empirical observations suggest that this design often struggles to effectively capture complex dynamic 3D scenes. Inspired by TensoRF~\cite{chen2022tensorf}, recent methods~\cite{cao2023hexplane,fridovich2023k,shao2023tensor4d} propose to utilize 4D volume factorization to represent dynamic 3D scenes. In particular, if we denote $XYZ$, $T$, and $F$ as the spatial resolution, temporal resolution, and feature size, HexPlane~\cite{cao2023hexplane} represents a 4D feature volume $\mathbf{D} \in \mathbb{R}^{XYZTF}$ as:
\begin{gather}
    \mathbf{D} = \sum_{r=1}^{R_1} \mathbf{M}_{r}^{XY} \circ \mathbf{M}_{r}^{XY} \circ \mathbf{v}_{r}^{1} + \sum_{r=1}^{R_2} \mathbf{M}_{r}^{XZ} \circ \mathbf{M}_{r}^{YT} \circ \mathbf{v}_{r}^{2} \\
    + \sum_{r=1}^{R_3} \mathbf{M}_{r}^{YZ} \circ \mathbf{M}_{r}^{XT} \circ \mathbf{v}_{r}^{3} \nonumber,
\end{gather}
where $\circ$ is outer product and each $\mathbf{M}_{r}^{AB}$ is a learned plane of features. For a 3D point at time $t$, its density and appearance feature can be quired from HexPlane using bilinear interpolations and vector-matrix product. The final color is then predicted through a tiny MLP that takes the appearance features and view direction as input. To train HexPlane, a combination of photometric loss and regularization terms, including Total Variational (TV) loss, are employed:
\begin{equation}
     \mathcal{L} = \sum_{\mathbf{r} \in \mathcal{R}, t \in \mathcal{M}} \Big\Vert \hat{C}(\mathbf{r},t) - C(\mathbf{r},t) \Big\Vert_2^{2} + \lambda_{reg} \mathcal{L}_{reg},
\end{equation}
where $\mathcal{R}$ is the set of all training rays and $\mathcal{M}$ is the time frame set.
